Discourse Structure in Machine Translation Evaluation

In this article, we explore the potential of using sentence-level discourse structure for machine translation evaluation. We first design discourse-aware similarity measures, which use all-subtree kernels to compare discourse parse trees in accordance with the Rhetorical Structure Theory (RST). Then, we show that a simple linear combination with these measures can help improve various existing machine translation evaluation metrics regarding correlation with human judgments both at the segment- and at the system-level. This suggests that discourse information is complementary to the information used by many of the existing evaluation metrics, and thus it could be taken into account when developing richer evaluation metrics, such as the WMT-14 winning combined metric DiscoTKparty. We also provide a detailed analysis of the relevance of various discourse elements and relations from the RST parse trees for machine translation evaluation. In particular we show that: (i) all aspects of the RST tree are relevant, (ii) nuclearity is more useful than relation type, and (iii) the similarity of the translation RST tree to the reference tree is positively correlated with translation quality.

==> sections/WMTexp.tex <==
% !TEX root = ../DiscoMTEval.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Discourse Structure in Machine Translation Evaluation
% Joty, Guzmán, Màrquez and Nakov
% QCRI, September 2014
%
% Section 5: DiscoTK Evaluation Metric
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Section~\ref{sec:ACLexp}, we experimented with two basic structures of the discourse tree, and we have shown that discourse information is complementary to the information sources used by state-of-the-art MT evaluation metrics.
In the present section, the goal is to build a strong, competitive evaluation metric. For this purpose, we explore three new discourse tree representations, in addition to \qcri \ and \qcril. We further combine the discourse scores with the metrics in Asiya, and we tune the weights of the combination on several WMT datasets. %The evaluation arena is the WMT14 shared Metrics Task \cite{machacek-bojar:2014:W14-33}.

%\paco{ In the previous sections, we have observed how both relation and nuclearity information in discourse trees is helpful for machine translation evaluation. Moreover, we observed how having lexicalized discourse trees have better lead to stronger metrics? 
%However, we would like to make this information available to the metric at all times. Also we would like to combine different metrics, because the stronger the better. Each metric looks at different aspects and it can contibute to a better score.}

%\sketch{Motivation: explore more representations of the discourse trees and try to produce a strong evaluation metric. Combination is needed. We follow the same learning of interpolation weights and usage of Asiya metrics for the combination. The evaluation arena is the WMT 14 task on translation evaluation.}

%\shafiq{We have shown discourse structure is complementary to state-of-the-art evaluation metrics using two basic structures of the DT. Now the goal is to build a strong evaluation metric combining the discourse-based metrics with others. For that, in addition to \qcri \ and \qcril, we explore three new DT representations.}

\subsection{Three New DT Representations}

%\lluis{This is copy\&pasted from the WMT paper. It has to be reduced to describe only the new tree representations not covered by Section~\ref{sec:measures}. Also Figure~\ref{fig:trees} has to be simplified accordingly (eliminate the cases from Figure 2). An alternative is to have a single Figure 2-3, but I believe I prefer it split in two.}

Figure~\ref{fig:trees} presents our three new representations of the discourse tree. The first one (\drLEX) shown in Figure \ref{fig:lex1}, is the direct output of the discourse parser, where the words of an EDU are grouped as children under the predefined EDU tag, constituting the leaves of the tree. The nuclearity statuses are attached to the EDU tags and to the relation labels. Note that \drLEX \ provides a more strict metric than \qcril \ described in Section \ref{sec:measures}. Unlike \qcril, \drLEX \ does not separate the skeleton of the tree from its labels. Therefore the tree kernel, when applied to this tree structure, does not give any partial credit to subtrees that match only on the structure or on the labels.  
  
\begin{figure*}[t]
	\begin{subfigure}{.7\linewidth}
	\centering 		
		\includegraphics [scale=0.65] {images/dr_lex_1_f.pdf}
	    \caption{DT for \drLEX}
	     \label{fig:lex1}
	\end{subfigure}	

	\begin{subfigure}{.7\linewidth}
	\centering
		 \includegraphics [scale=0.65] {images/dr_lex_1_1.pdf}
	    \caption{DT for \drLEXoo}
	     \label{fig:lex1.1}
	\end{subfigure}

	\begin{subfigure}{.7\linewidth}
	\mbox{\hspace{-0.48cm}
		 \includegraphics [scale=0.40] {images/dr_lex_2_1.pdf}}
	    \caption{DT for \drLEXe}
	     \label{fig:lex2.1}
	\end{subfigure}
\caption{Three new representations of the discourse tree for the sentence: \emph{``The new organisational structure will also allow us to enter the market with a joint offer of advertising products, to better link the creation of content for all the titles published and, last but not least, to continue to streamline significantly the business management of the company,'' added Cermak.} 
To avoid visual clutter, (b) and (c) show alternative representations only for the highlighted subtree in (a).}
\label{fig:trees}
\end{figure*}
  
  
Although tree kernels applied to \qcril \ and \drLEX \ find matches at the word level (using dummy leaves),\footnote{We include dummy leaves in all our lexicalized versions of a discourse tree.} the words are compared in a bag-of-words fashion, i.e., if the two trees share a common word, the kernel will find a match regardless of its position in the tree. Therefore, a word that has occurred in an EDU with nuclearity status \emph{Nucleus} in one tree could be matched with the same word under a \emph{Satellite} status in the other tree. In other words, the tree kernel defined on these representations is insensitive to the nuclearity statuses and the relation labels under which the words are matched. \drLEXoo, an extension of \drLEX, and \drLEXe, an extension of \qcril, are sensitive to these variations at the lexical level.  \drLEXoo \ and \drLEXe, as shown in Figures \ref{fig:lex1.1} and \ref{fig:lex2.1}, propagate the nuclearity statuses and/or the relation labels to the lexical items by including three more subtrees at the EDU level: one for nuclearity (subtree rooted at the LEX:NUC tag), one for relation labels (subtree rooted at the LEX:REL tag), and one for both nuclearity and relation labels (subtree rooted at the LEX:NUC:REL tag).  

%\shafiq{Should we use figures with the same example as in Section 2?}
%\preslav{Ideally, we should have the same examples in the entire paper, which would allow for more direct comparison. But then, I guess it can remain like this for the initial submission, unless somebody is keen to redraw the trees...}

%  Coherence relations, such as \emph{Attribution}, \emph{Elaboration}, and \emph{Enablement}, between adjacent text spans constitute the internal nodes of the tree. Like the EDUs, the nuclearity statuses of the larger discourse units are attached to the relation labels.


\subsection{Metric Combination}

We experimented with 
%two metric combinations:
\discolight, which combines the five discourse-based metrics,
and
\discoparty, which further adds the Asiya metrics to the combination.
We tuned the relative weights of the individual metrics in a combination using the maximum entropy learning framework, as we described in Subsection~\ref{DataPreprocess}.
%
%\lluis{The following is the WMT14 text; we have to adapt it to include also the results on WMT14 datasets (and maybe a comparison to the other participant systems; small table of results); the text can be slightly reduced. Also, it has to be added a blurb summarizing the following \emph{Post-processing} paragraph}
%
Note that our discourse-based metrics, especially \dr, tend to produce many ties when there is no enough information to perform complete discourse analysis. This contributes to lower $\tau$ scores for \discolight. To alleviate this issue, we used a simple tie-breaking strategy, in which ties between segment scores for different systems are resolved by using perturbations proportional to the global system-level scores produced by the same metric.
%,
%i.e., $x'^{seg}_{sys}$= $x^{seg}_{sys}+\epsilon*\sum_s x^s_{sys}$.
%Here, $\epsilon$ is automatically chosen to avoid collisions with %other
%scores not involved in the tie.
This post-processing is not part of the metric; we applied it to our 
%official 
segment-level submission to the \wmtf\ Metrics task.

%, which relies solely on discourse.


% We have two main versions:
% \discolight, which combines the five DR-based metrics,
% and
% \discoparty, which further adds the Asiya metrics.
% \medskip

% \noindent\lluis{The WMT paper has a detailed description on the combination, learning, Asiya metrics from Disco party, etc. This is included but commented in the current \emph{WMTexp.tex} file. I guess that all this stuff is covered already in Section~\ref{sec:setting} of this paper; we only have to recall this and point to the appropriate section.}

% \preslav{Well, this is true, but we now want to say that we now have five, not two DR-* metrics.}

%%%%%%%%%%%%%%%%%%%%%%%%%% from WMT14 paper: we can skip it and refer to section 4
%\subsection{\discolight}
%
%In the previous section, we have presented several discourse tree representations that can be used to compare the output of a machine translation system to a human reference. Each representation stresses a different aspect of the discourse tree.
%
%In order to make our estimations more robust, we propose \discolight,
%a metric that takes advantage of all the previous discourse representations by linearly interpolating their scores.
%Here are the processing steps needed to compute this metric:
%
%
%\noindent\Ni Parsing:
%We parsed each sentence in order to produce discourse trees for the human references and for the outputs of the systems.
%
%\noindent\Nii Tree enrichment/simplification:
%For each sentence-level discourse tree,
%we generated the five different tree representations: \dr, \drLEX, \drLEXoo, \drLEXto, \drLEXtt.
%
%\noindent\Niii Estimation:
%We calculated the per-sentence similarity scores between tree representations of the system hypothesis and the human reference using the extended convolution tree kernel as described in the previous section. To compute the system-level similarity scores, we calculated the average sentence-level similarity;
%note that this ensures that our metric is ``the same'' at the system and at the segment level.
%
%\noindent\Niv Normalization:
%In order to make the scores of the different representations comparable,
%we performed a $\min$--$\max$ normalization\footnote{Where $x'=(x-\min)/(\max-\min)$.}
%%using the maximum and minimum similarity scores for each representation across all segments and systems,
%for each metric and for each language pair.
%
%\noindent\Nv Combination:
%Finally, for each sentence,
%we computed \discolight~ as the
%%uniform linear interpolation
%average of the normalized similarity scores
%of the different representations.
%For system-level experiments,
%we performed linear interpolation of system-level scores.
%
%
%%\subsection{\discoparty~: Based on metric combination}
%\subsection{\discoparty}
%
%One of the weaknesses of the above discourse-based metrics is that they use unigram lexical information,
%which does not capture reordering.
%%Furthermore, we have previously shown \cite{discoMT:acl2014}
%%that discourse information can help improve many MT evaluation metrics.
%Thus, in order to make more informed and robust estimations,
%we extended \discolight \ with the composing metrics of the \asiya's ULC~metric~\cite{AsiyaMTjournal:2010},
%which is a uniform linear combination of twelve individual metrics
%and was the best-performing metric at the system and at the segment levels
%at the WMT08 and WMT09 metrics tasks.
%
%In order to compute the individual metrics from ULC,
%we used the \asiya\ toolkit,\footnote{http://nlp.lsi.upc.edu/asiya/}
%%\cite{AsiyaPBML:2010},
%but we departed from \asiya's ULC
%by replacing TER and Meteor with newer versions thereof
%that take into account synonymy lookup and paraphrasing (`TERp-A' and `Meteor-pa' in \asiya's terminology).
%%
%We then combined the five components in \discolight\ and the twelve individual metrics from ULC;
%we call this combination \discoparty.
%
%We combined the scores using linear interpolation in two different ways:
%
%\noindent\Ni \emph{Uniform combination} of $\min$-$\max$ normalized scores at the segment level.
%We obtained system-level scores by computing the average over the segment scores.
%
%\noindent\Nii \emph{Trained interpolation at the sentence level}.
%We determined the interpolation weights for the above-described combination of 5+12 = 17 metrics
%using a pairwise learning-to-rank framework and classification with logistic regression,
%as we had done in \cite{discoMT:acl2014}.
%We obtained the final test-time sentence-level scores by passing the interpolated raw scores through a sigmoid function.
%In contrast, for the final system-level scores, we averaged the per-sentence interpolated raw scores.
%
%We also tried to learn the interpolation weights at the system level,
%experimenting with both regression and classification.
%However, the amount of data available for this type of training was small,
%and the learned weights did not perform significantly better than the uniform combination.

%------------------------ Experiments
\subsection{Experiments}

\noindent Below we present the results of our experiments with the different \disco\ metric variants and using various tuning datasets from \wmt\ metrics shared tasks, i.e., 2011, 2012 and 2013.
%In particular, we processed and used those of 2011, 2012 and 2013.
From Section~\ref{sec:ACLexp} above, we already know that the tuned metrics perform well on cross-validation for the same-year dataset. We further know that tuning can be performed by concatenating the available data from all the into-English language pairs from a given year, which yields better results than tuning separately for each language pair. Here, we investigate in more depth \Ni whether the tuned metrics generalize well to new datasets, and \Nii the effect of tuning on concatenated datasets from different years.

% Additionally, we test the effect of tuning on concatenated datasets from different years in order to obtain larger tuning datasets.

Table~\ref{tab:results} shows the results.
%Several additional experiments and combinations were carried out, but not shown due to space limitations.
We evaluated the performance of the metrics on the \wmtt\ and \wmth\ datasets both at the segment and at the system level, and we used \wmte\ as an additional tuning dataset. We tried various combinations of datasets for tuning.
%We measured the performance of the metrics in terms of correlation with human judgements. At the segment level, we evaluated using Kendall's Tau ($\tau$),
%recalculated following the \wmtf\ official Kendall's Tau implementation.
%At the system level, we used Spearman's rank correlation ($\rho$) and Pearson's correlation coefficient ($r$). %in the case of system-level evaluation.
%In all cases, 
We averaged the results over all into-English language pairs. The symbol `$\varnothing$' marks the untuned versions of our metrics, i.e., applying a uniform linear combination of the individual metrics in the metric combination.

We trained the tuned versions of the \disco\ measures using different datasets (\wmte, \wmtt\ and \wmth)
in order to study cross-corpora generalization and the effect of training dataset size.
The symbol `+' stands for concatenation of datasets. %We trained the tuned versions at the segment level using Maximum Entropy classifiers for pairwise ranking. 
For the sake of comparison, the first group of rows contains the results of the best-performing metrics at the \wmtt\ and \wmth\ metrics shared tasks and the last group of rows contains the results of the \asiya\ combination of metrics, i.e.,~\discoparty\ without the discourse components. %, at the segment and at the system levels.


\begin{table*}[t]
\small
\begin{center}
\begin{tabular}{rccccccc}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\bf Segment Level} & \multicolumn{4}{c}{\bf System Level}\\
%\cline{3-4}\cline{5-8}
\multicolumn{2}{c}{} & \wmtt & \sc \wmth & \multicolumn{2}{c}{\wmtt} & \multicolumn{2}{c}{\wmth}\\
%\cline{3-3}\cline{4-4}\cline{5-6}\cline{7-8}
\bf Metric & \bf Tuning & \multicolumn{1}{c}{$\tau$} & \multicolumn{1}{c}{$\tau$} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{$r$} & \multicolumn{1}{c}{$\rho$} & \multicolumn{1}{c}{$r$}\\
\hline
 \sempos & na & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 0.902 & 0.922 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}\\
 \spede  & na & 0.254 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}\\
 {\sc Meteor-wmt13} & na & \multicolumn{1}{c}{--} & 0.264 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 0.935	& {\bf 0.950}\\
\hline
            & $\varnothing$ & 0.171 & 0.162 & 0.884 & 0.922 & 0.880 & 0.911\\
            & \wmte         & 0.207 & 0.201 & 0.860 & 0.872 & 0.890 & 0.909\\
\discolight & \wmtt         & --    & 0.200 & --    & --    & 0.889 & 0.910\\
            & \wmth         & 0.206 & --    & 0.865 & 0.871 & --    & --\\
            & \wmte+12      & --    & 0.197 & --    & --    & 0.890 & 0.910\\
            & \wmte+13      & 0.207 & --    & 0.865 & 0.871 & --    & --\\
\hline
            & $\varnothing$ & 0.257 & 0.231 & 0.907 & 0.915 & {\bf 0.941} & 0.928\\
            & \wmte         & 0.302 & 0.282 & {\bf 0.915} & {\bf 0.940} & 0.934 & 0.946\\
\discoparty & \wmtt         & --    & 0.284 & --    & --    & 0.936 & 0.940\\
            & \wmth         & {\bf 0.305} & --    & 0.912 & 0.935 & -- & --\\
            & \wmte+12      & --    & {\bf 0.289} & -- & -- & 0.936 & 0.943\\
            & \wmte+13      & 0.304 & --    & 0.912 & 0.934 & -- & --\\
\hline

 & $\varnothing$            & 0.273 & 0.252 & 0.899 & 0.909 & 0.932 & 0.922\\
            & \wmte         & 0.301 & 0.279 & 0.913 & 0.935 & 0.934 & 0.944\\
{\sc \asiya}            & \wmtt         & --    & 0.277 & --    & --    & 0.932 & 0.938\\
& \wmth         & 0.303 & --    & 0.908 & 0.932 & --    & --\\
            & \wmte+12      & --    & 0.277 & --    & --    & 0.934 & 0.940\\
            & \wmte+13      & 0.303 & --    & 0.908 & 0.933 & --    & --\\

\hline
\end{tabular}
\end{center}
\caption{\label{tab:results}Results at the segment and at the system level for the \disco\ metrics: tuning on the \wmte, \wmtt, and \wmth datasets, and testing on \wmtt\ and \wmth. For comparison, we also include some other metrics in the top and in the bottom rows.}
%\vspace{-5pt}
\end{table*}

Several conclusions can be drawn from Table~\ref{tab:results}.
First, \discoparty\ is better than \discolight\ in all settings, indicating that the discourse-based metrics are very well complemented by the heterogeneous metric set from \asiya. 
%\discolight\ achieves competitive scores at the system level (which would put the metric among the best participants in \wmtt\ and \wmth); however, as expected, it is not robust enough at the segment level. 
On the other hand, the tuned versions of \discoparty\ are very competitive and improve over the already strong \asiya\ in each configuration both at the segment- and the system-level. The improvements are small but consistent, showing that using discourse information improves the correlation with human judgments.

Focusing on the results at the segment level, it is clear that the tuned versions offer an advantage over the simple uniform linear combinations. Interestingly, for the tuned variants of the metric, given a test set, the results are consistent across all tuning datasets, which rules out over-fitting. Thus, we can conclude that the generalization of the tuning is very good, and there is no overfitting.
%This result aligns well with what we observed in our previous studies~\cite{discoMT:acl2014}. 
Learning with more data (\wmte+12 or \wmtt+13) does not seem to help much, but it does not hurt performance either. 

Overall, the Kendall's $\tau$ correlation results obtained with the tuned \discoparty\ metric are much better than the best results of any participant metric at \wmtt\ and \wmth\ (20.1\% and 9.5\% relative improvement, respectively).

At the system level, we observe that tuning the \discolight\ metric is not helpful (results are actually slightly lower), while tuning the more complex \discoparty\ metric yields slightly better results. %At the system level,

The scores of our best metric are higher than those of the best participants in \wmtt\ and \wmth\, according to Spearman's $\rho$, which was the official metric in those years.
%
Overall, our metrics are comparable to the state-of-the-art at the system level. The differences between Spearman's $\rho$ and Pearson's $r$ coefficients are not dramatic, with $r$ values being always higher than $\rho$.
%Note also that the tuned \discoparty\ is better than the tuned \asiya\ for all tuning conditions and all evaluation datasets,
%at both the segment- and the system-level.

Given the above results, we submitted the following runs to the \wmtf\ Metrics shared task: \Ni \discoparty\ tuned on the concatenation of datasets \wmte+12+13, as our primary run; \Nii Untuned \discoparty, to verify that we are not over-fitting the training set; and \Niii Untuned \discolight, to see
the performance of a metric using only discourse structures and word unigrams.
%how far we can get with a simple combination metric based only on discourse structures and word unigrams.

The results for the \wmtf\ Metrics shared task have shown that our primary run, \discoparty\ tuned,
was the best-performing metric both at the segment and at the system level, among a set of 16 and 20 participants, respectively~\cite{machacek-bojar:2014:W14-33}.
%Not surprisingly, the untuned \discoparty \ yielded slightly worse results than its tuned counterpart,
%which confirms that there was no over-fitting during tuning.
This metric yielded much better results than its untuned counterpart,
confirming the importance of weight tuning and the absence of over-fitting during tuning.
Finally, the untuned \discolight\ achieved expectedly slightly worse results for all language pairs, except for Hindi-English, for which the results were much lower.
System translations for Hindi-English resembled a ``word salad'' in most cases, and were very hard to discourse-parse accurately.\footnote{Note that the Hindi-English language pair caused a similar problem for a number of other metrics at the \wmth\ Shared Task competition that relied on linguistic analysis.}
%\preslav{Do we want to show more results about WMT14?}

\begin{table*}[t]
\small
\begin{center}
\begin{tabular}{@{ }lccccc@{ }}
\bf System & \bf fr-en & \bf de-en & \bf hi-en & \bf cs-en & \bf ru-en\\
\hline
\discoparty   & \bf 0.433 & \bf 0.380 & 0.434      & \bf 0.328 & \bf 0.355 \\
Best at \wmtf & 0.417     & 0.345    & \bf 0.438  & 0.284  & 0.336 \\
              & +0.016              & +0.035              & -0.004              & +0.044 & +0.019\\
\hline
\end{tabular}
\end{center}
\caption{\label{tab:WMT14:comparetothebest:segment}Comparing our tuned metric to the best rivaling metric at \wmtf, for each individual language pair (this best rival differs across language pairs) at the segment-level using Kendall's $\tau$.}

%\vspace{-5pt}
\end{table*}

% \begin{table*}[t]
% \small
% \begin{center}
% \begin{tabular}{@{ }lccccc@{ }}
% \bf System & \bf fr-en & \bf de-en & \bf hi-en & \bf cs-en & \bf ru-en\\
% \hline
% \discoparty   & \bf 0.433 $\pm$ 0.012 & \bf 0.380 $\pm$ 0.013 & 0.434 $\pm$ 0.013     & \bf 0.328 $\pm$ 0.015 & \bf 0.355 $\pm$ 0.011\\
% Best at \wmtf & 0.417 $\pm$ 0.013     & 0.345 $\pm$ 0.014     & \bf 0.438 $\pm$ 0.013 & 0.284 $\pm$ 0.015 & 0.336 $\pm$ 0.011\\
%               & +0.016              & +0.035              & -0.004              & +0.044 & +0.019\\
% \hline
% \end{tabular}
% \end{center}
% \caption{\label{tab:WMT14:comparetothebest:segment}Comparing our tuned metric to the best rivaling metric at \wmtf, for each individual language pair (this best rival differs across language pairs) at the segment-level using Kendall's $\tau$.}
% %\vspace{-5pt}
% \end{table*}


% \begin{table*}[t]
% \small
% \begin{center}
% \begin{tabular}{@{ }lccccc@{ }}
% \bf System & \bf fr-en & \bf de-en & \bf hi-en & \bf cs-en & \bf ru-en\\
% \hline
% \discoparty   & 0.977 $\pm$ 0.009 & \bf 0.943 $\pm$ 0.020 & 0.956 $\pm$ 0.007 & 0.975 $\pm$ 0.031 & \bf 0.870 $\pm$ 0.022\\
% Best at \wmth & \bf 0.981 $\pm$ 0.008 & 0.935 $\pm$ 0.022 & \bf 0.976 $\pm$ 0.006 & \bf 0.993 $\pm$ 0.018 & 0.856 $\pm$ 0.023\\
%               &-0.004             &+0.008             & -0.020 & -0.018 & +0.014\\
% \hline
% \end{tabular}
% \end{center}
% \caption{\label{tab:WMT14:comparetothebest:system}Comparing our tuned metric to the best rivaling metric at \wmtf, for each individual language pair (this best rival differs across language pairs) at the system-level using Person's correlation.}
% %\vspace{-5pt}
% \end{table*}

Table~\ref{tab:WMT14:comparetothebest:segment} shows a comparison at the segment level of our tuned metric \discoparty \ to the best rivaling metric at \wmtf, for each individual language pair, using Kendall's $\tau$.\footnote{Note that here we report the \wmtf\ version of Kendall's $\tau$, which differs slightly from the version that was used in previous years; see \cite{machacek-bojar:2014:W14-33} for detail.} 
Note that this best rival differs across language pairs, e.g., for fr-en, hi-en, and cs-en it is \textsc{beer}, for de-en it is \textsc{upc-stout}, and for ru-en it is \textsc{REDcombSent}. We can see that our metric outperforms this best rival for four of the language pairs 
%and this improvement is statistically significant\footnote{According to the empirical confidence intervals of Kendall's $\tau$, which were obtained through bootstrap resampling.} 
in all four cases. The only exception is hi-en, where the best rival performs slightly better.
%, but the difference is not statistically significant.

In absolute terms, we do not observe any clear correlation between the quality of the translation hypotheses and the performance of our metric. 
While our tuned \discoparty \ metric  expectedly achieves much higher $\tau$ for fr-en ($\tau$=0.433) compared to cs-en, ru-en, and de-en ($\tau$ of 0.328, 0.355 and 0.380, respectively), for hi-en it performs virtually the same as for fr-en: 0.433 vs. 0.434.
However, in relative terms, we see that our metric is outperformed by the best rival for hi-en (this is the only system that could beat our tuned \discoparty), which suggests that the linguistically-heavy components of our \discoparty\ (discourse parsing, syntactic parsing, semantic role labeling, etc.) may suffer from the common ungrammaticality of the translation hypotheses for hi-en, while other, less linguistically-heavy metrics seem to be more robust in such cases.

\begin{figure}[htbp!]
\centering
\pgfplotsset{width=10cm,compat=1.3}
\begin{tikzpicture}
\begin{axis}[
footnotesize,
symbolic x coords={BLEU, NIST, TER, TERp-A, ROUGE-W, METEOR-ex, METEOR-pa, METEOR-st, METEOR-sy, DP-HWCM-c-4, DP-HWCM-r-4, DP-Or*, CP-STM-4, SR-Or*, SR-Mr, SR-Or,DR-Or*,DR-Orp*, DR-NOLEX, DR-LEX, DR-LEX$_e$, DR-LEX-1,DR-LEX-1.1},
ybar=1pt, %space between ybars
bar width=5pt,
ymin=0,   %ybar starts from
width=13.5cm,
enlarge x limits=0.02,
height=6cm,
%nodes near coords,
xlabel={Metrics},
ylabel={Coefficients},
x tick label style={rotate=90,anchor=east, font=\footnotesize},
yticklabel style={/pgf/number format/fixed},
xtick=data]

\addplot [fill=blue]
coordinates {(BLEU, 0.19) (NIST, 0.02) (TER, 0.03) (TERp-A, 0.49) (ROUGE-W, 0.25) (METEOR-ex, 0.16) (METEOR-pa, 0.33) (METEOR-st, 0.15) (METEOR-sy, 0.08) (DP-HWCM-c-4, 0.02) (DP-HWCM-r-4, 0.04) (DP-Or*, 0.14) (CP-STM-4, 0.19) (SR-Or*, 0.07) (SR-Mr, 0.06) (SR-Or, 0.04) (DR-Or*, 0.01) (DR-Orp*, 0.18) (DR-NOLEX, 0.08) (DR-LEX, 0.10) (DR-LEX-1, 0.22)  (DR-LEX-1.1, 0.10) (DR-LEX$_e$, 0.13)};

%\legend{Multi-sentential, Intra-sentential}
\end{axis}
\end{tikzpicture}
\caption{Absolute coefficient values after tuning the \discoparty\ metric on the WMT11+12+13 dataset.}
\label{fig:freq}
\end{figure}

Finally, we show in Figure~\ref{fig:freq} the weights for the individual metrics combined in \discoparty\ after tuning on the combined WMT11+12+13 dataset. The horizontal axis displays all the individual metrics involved in the combination. The first block of metrics (from BLEU to DR-Orp*) consists of the 18 \asiya\ metrics described in~\ref{subsubsec:asiya}. The last five (from \dr \ to \drLEXoo) metrics are the metric variants based on discourse trees. Note that all metric scores are passed through a \emph{min-max} normalization step to put them in the same scale before tuning their relative weights.
 
We can see in Figure~\ref{fig:freq} that most of the metrics involved in the metric combination play a significant role, the most important ones being TERp-A, METEOR-pa (paraphrases), and ROUGE-W. Some metrics accounting for syntactic and semantic information also get assigned relatively high weights (\hbox{DP-Or*}, CP-STM-4, and DR-Orp*). More interestingly, all five variants of our discourse metric received moderately-high weights,
with the four variants of our discourse metrics with lexical information (\qcril) being more important. In particular, \drLEX\ has the fourth highest absolute weight in the overall combination. This confirms once again the importance of using discourse information for machine translation evaluation.


==> tables/tab-results-wmt12-seg-tuned.tex <==

\begin{table}[t]
\begin{center}
{\small\begin{tabular}{@{}l@{}rrrr@{ }@{ }r}
%\cline{2-5}

&&& \multicolumn{3}{c}{\bf Tuned}\\
\cmidrule{4-6}
&\bf Metrics & \bf Orig.  & & +\sqcri & +\sqcril\\
\toprule
\multirow{ 2}{*}{\bf I}&\qcri  & -.433 & -- & -- & --\\
&\qcril &  .133 & -- & -- & -- \\
\hline
\multirow{ 9}{*}{\bf II}&\spede  & .254 & -- & \it .253 &  .254\\
&\meteor & .247 & -- & \bf .250 & \bf .251\\
&\amber  & .229 & -- & \bf .230 & \bf .232 \\
&\simpbleu &  .172 & -- & \bf .181 & \bf .199 \\
&\terrorcat & -.186 & -- & \bf .181 & \bf .196\\
&\xen & .165 & -- & \bf .175 & \bf .194 \\
&\posf & .154 & -- & \bf .160 & \bf .201\\
&\word & .153 & -- & \bf .161 & \bf .189\\
&\block & .074 & -- & \bf .087 & \bf .150\\
\hline
\multirow{ 4}{*}{\bf III}&\nist & .214 & -- & \bf .222 & \bf .224\\
&\rouge & .185 & -- & \bf .196 & \bf .218\\
&\ter & .217 & -- & \bf .229 & \bf .246\\
&\bleu & .185 & -- & \bf .189 & \bf .194\\
\hline
\multirow{ 6}{*}{\bf IV}&\lex & .254 & .266 & \bf .269 & \bf .270 \\
&\syn & .177 & .229 & .228 & \bf .232 \\
&\srl & -.023 & -.004 & \bf .039 & \bf .181 \\
&\dis & .134 & .146 & \bf .179 & \bf .202 \\
&\asiyaix & .254 & .295 & .295 & .295 \\
&\asiyaall & .268 & .296 & .295 &  .295\\
\midrule
&\bf average & .165 & & .201 & .222\\
&\bf diff.    &      & & \bf +.036 & \bf  +.057\\
\bottomrule
\end{tabular}}
\end{center}
\caption{\label{tab:results-wmt12-seg-tuned}Results on WMT12 at the segment-level: tuning with cross-validation on WMT12. Kendall's $\tau$ with human judgments. 
%\lluis{Tables 3 and 4 can be pasted in a single table with more columns. I include a draft below...}
%\preslav{I like the combined table.}}
\vspace{-5mm}
\end{table}







==> tables/tab-results-wmt12-seg.tex <==

\begin{table}[t]
\begin{center}
{\small\begin{tabular}{@{}l@{}rrr@{ }@{ }r}

&\bf Metrics &  & +\sqcri & +\sqcril \\
\toprule
\multirow{ 2}{*}{\bf I}&\qcri & -.433 & -- & -- \\
&\qcril & .133 & -- & -- \\
\midrule
\multirow{ 9}{*}{\bf II}&\spede & .254 & \it .190 & \it .223 \\
&\meteor & .247 & \it .178 & \it .217 \\
&\amber & .229 & \it .180 & \it .216 \\
&\simpbleu & .172 & \it .141 & \bf .191\\
&\xen & .165 & \it .132 & \bf .185 \\
&\posf & .154 & \it .125 & \bf .201 \\
&\word & .153 & \it .122 & \bf .181 \\
&\block & .074 & \it .068 & \bf .151 \\
&\terrorcat & -.186 & \bf -.111 & \bf -.104 \\
\midrule
\multirow{ 4}{*}{\bf III}&\bleu & .185 & \it .154 & \bf .190 \\
&\nist & .214 & \it .172 & \it .206 \\
&\rouge & .185 & \it .144 & \bf .201 \\
&\ter & .217 & \it .179 & \bf .229 \\
\midrule
%\multirow{ 6}{*}{\bf IV}&\lex & .254 & \it .237 & \it .253 \\
%&\syn & .177 & \it .169 & \bf .191 \\
%&\srl & -.023 & \bf .015 & \bf .161 \\
%&\dis & .134 & \bf .152 & \bf .197 \\
%&\asiyaix & .254 & \it .250 & \bf .258 \\
%&\asiyaall & .268 & \it .265 & \bf .270 \\
%\midrule
&\bf average & .165 & \it .145 & \bf .190 \\
&\bf diff. & & \it -.019 & \bf +.026 \\
\bottomrule
\end{tabular}}
\end{center}
\caption{\label{tab:results-wmt12-seg}Results on WMT12 at the segment-level. Kendall's $\tau$ with human judgments.}
\vspace{-5mm}

\end{table}

==> tables/tab-results-wmt12-seg_copy.tex <==

\begin{table}[t]
\begin{center}
{\small\begin{tabular}{@{}l@{}rrr@{ }@{ }r}

&\bf Metrics &  & +\sqcri & +\sqcril \\
\toprule
\multirow{ 2}{*}{\bf I}&\qcri & -.433 & -- & -- \\
&\qcril & .133 & -- & -- \\
\midrule
\multirow{ 9}{*}{\bf II}&\spede & .254 & \it .190 & \it .223 \\
&\meteor & .247 & \it .178 & \it .217 \\
&\amber & .229 & \it .180 & \it .216 \\
&\simpbleu & .172 & \it .141 & \bf .191\\
&\xen & .165 & \it .132 & \bf .185 \\
&\posf & .154 & \it .125 & \bf .201 \\
&\word & .153 & \it .122 & \bf .181 \\
&\block & .074 & \it .068 & \bf .151 \\
&\terrorcat & -.186 & \bf -.111 & \bf -.104 \\
\midrule
\multirow{ 4}{*}{\bf III}&\nist & .214 & \it .172 & \it .206 \\
&\rouge & .185 & \it .144 & \bf .201 \\
&\ter & .217 & \it .179 & \bf .229 \\
&\bleu & .185 & \it .154 & \bf .190 \\
\midrule
\multirow{ 6}{*}{\bf IV}&\lex & .254 & \it .237 & \it .253 \\
&\syn & .177 & \it .169 & \bf .191 \\
&\srl & -.023 & \bf .015 & \bf .161 \\
&\dis & .134 & \bf .152 & \bf .197 \\
&\asiyaix & .254 & \it .250 & \bf .258 \\
&\asiyaall & .268 & \it .265 & \bf .270 \\
\midrule
&\bf average & .165 & \it .145 & \bf .190 \\
&\bf diff. & & \it -.019 & \bf +.026 \\
\bottomrule
\end{tabular}}
\end{center}
\caption{\label{tab:results-wmt12-seg}Results on WMT12 at the segment-level. Kendall's $\tau$ with human judgments.}
\vspace{-5mm}

\end{table}
